Meta Mirror Descent: Optimiser Learning for Fast Convergence

Optimisers are an essential component for training machine learning models, and their design influences learning speed and generalisation. Several studies have attempted to learn more effective gradient-descent optimisers via solving a bi-level optimisation problem where generalisation error is minimised with respect to optimiser parameters. However, most existing optimiser learning methods are intuitively motivated, without clear theoretical support. We take a different perspective starting from mirror descent rather than gradient descent, and meta-learning the corresponding Bregman divergence. Within this paradigm, we formalise a novel meta-learning objective of minimising the regret bound of learning. The resulting framework, termed Meta Mirror Descent (MetaMD), learns to accelerate optimisation speed. Unlike many meta-learned optimisers, it also supports convergence and generalisation guarantees and uniquely does so without requiring validation data. We evaluate our framework on a variety of tasks and architectures in terms of convergence rate and generalisation error and demonstrate strong performance.

==> 4_experiments_old.tex <==
\section{Experiments}
In this section, we demonstrate the properties of the proposed algorithm and illustrate the performances of the learned optimiser in a variety of tasks. 
\subsection{Meta-Quadratic optimisation}
We creat a 2D meta-Quadratic optimisation problem, satisfying all the assumptions for developing \ourModel{}, to setup a deal environment to test our algorithm and compete with other commonly used first-order optimiser in the deep learning community. The tasks can be sampled from a same distribution by: 
\begin{align}
 \min x^T Q x - b^T x 
\end{align}
where Q is sample from a contracated Gaussian distribution to create a very flat function contour a long the x-axis and b is sample from another Gaussian distribution with the mean and varience. We sample a group of tasks to learn an optimiser with one diagnoal Mahalanobis. Due to the specific definitation of Q, the Quadratic problem sampled from the task distribution are all convex and contain very flat function contour. 
\begin{figure*}[t]
\centering
\includegraphics[width=0.24\textwidth]{meta_quadra/task1/row1_MetaMD.eps}
\includegraphics[width=0.24\textwidth]{meta_quadra/task1/row1_SGD.eps}
\includegraphics[width=0.24\textwidth]{meta_quadra/task1/row1_SGD-M.eps}
\includegraphics[width=0.24\textwidth]{meta_quadra/task1/row1_Adam.eps}
\includegraphics[width=0.24\textwidth]{meta_quadra/task2/row2_MetaMD.eps}
\includegraphics[width=0.24\textwidth]{meta_quadra/task2/row2_SGD.eps}
\includegraphics[width=0.24\textwidth]{meta_quadra/task2/row2_SGD-M.eps}
\includegraphics[width=0.24\textwidth]{meta_quadra/task2/row2_Adam.eps}
\caption{Top Rwo: Meta-test performance of the learned \ourModel{}. Bottom: the performance of the competiters, from left to right: SGD, SGD-M, Adam, RMSprop, on the same setting. }
\label{fig:meta_quadr_2d}
\end{figure*}
After meta-training, we deploy \ourModel{} and the competiters on the same setting. To make fair comprisons, optimisers are initialised in the same position and the free parameters are updated until reaching the global minima. The optimisation process of all the optimisers are shown in Figure~\ref{fig:meta_quadr_2d}. It can be noticed that, more detials can be found in Appendix.


\subsection{Rosenbrock function}
We also test our algorithm on the Rosebrock function, a non-convex function which is commonly used as a testbed for the optimisation algorithm. In this setting, we set the training iteration as 500, and carefully running tunning the learning for all the competiters, including Adam, SGD, SGD-M, RMSprop. The optimisation trajectories of each competiter and \ourModel{} are give in Figure~\ref{fig:rosenbrock_fuc}.
\begin{figure}[t]
\centering
\includegraphics[width=0.49\columnwidth]{rosenbrock_plot/SGD-M_.eps}
\includegraphics[width=0.49\columnwidth]{rosenbrock_plot/Adam_.eps}
\includegraphics[width=0.49\columnwidth]{rosenbrock_plot/RMSprop_.eps}
\includegraphics[width=0.49\columnwidth]{rosenbrock_plot/MetaMD_.eps}
\caption{The optimisation trajecotries for solving the Rosenbrock function producded by different optimisers.}
\label{fig:rosenbrock_fuc}
\end{figure}
In order to show the fast convergence properties of \ourModel{}, we limite the optimisation step to 500. 

\subsection{Short and Long Horizon with MLP and RotatedMNIST}
Ideally, we want to train the base model by the learnable optimiser from scratch until it converges in the inner loop to make the optimiser observe the whole training process, then the updating information carried by the hypergradient is comprehensive for the gradient computation of the objective function in the outer loop. However, it will be very expensive and inefficient if the base model is a deep neural network, such as ResNet~\cite{}, WideResNet~\cite{}. In addition, even though the forward mode differentiation and the parameterisation of $\phi$ function solve hypergradient computation problem, but still if the inner loop optimisation is very long, the hypergradient may vanish and explode. To alleviate this problem, we assume when T is large enough so that $\theta_T$ is able to approximate $\theta_*$ in the large scale problem. To analysis the impact of the short horizons we test the algorithm on a variety of models, including linear model, 2-layer MLP and 3-layer MLP and RotatedMNIST. There are six domains of datasets in RotatedMNIST with different rotation angles on the MNIST dataset. In the meta-train stage, we use five of them and hold one domain out on the meta-test stage for testing the learned optimiser. We explore the short horizon by setting the inner loop in several relatively small iterations and also compare the learned optimiser with that learned from the long horizon.
Then we can expect that the gradient of the objective function with respect to the free parameters is zero when it reach the global optimum. In practice, the stop criteria for all the optimisers is set as $||g||_2 \leqslant \epsilon$, and $\epsilon$ is 0.001.
For the SGD, SGD-M and RMSprop, we sweep over the learning rates $\{0.1, 0.05, 0.01, 0.005, 0.001\}$ and weight decay parameters of $\{ 0.001, 0.0001, 0.0005\}$. In terms of Adam, we do grid seach over the learn rates $\{0.3, 0.2, 0.1, 0.01, 0.001\}$ and wegith decay $\{0.001, 0.0001, 0.0005\}$. In addition, it will be difficult to tune the hyperparameters for the competiters for each individual task, instead for each tyep of architectures, the hyperamters are tuned accoridng to the mean validation performance over all the domains, which is valid because the domain shift is not significatn among them. We leave the development of efficienty inner loop training with long horizon with deep base model in the future work.

\begin{table*}[t]
\centering
\caption{\textbf{RotatedMNIST with MLPs, test Accuracy/(training iteration) (\%)}} 
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{ l | l | c c c c c c}
\toprule
 &Method & 0 & 15 & 30 & 45 & 60 & 75 \\
\cmidrule{1-8}
\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{1-Layer MLP}}}
&SGD                                                                & 84.92 (1383) & 86.89 (1790) & 86.38 (1674) & 86.55 (1499) & 86.85 (1644) & 85.39 (1814) \\
&SGD +M09                                                           & 84.75  (192) & 86.50  (200) & 87.10  (223) & 87.10  (179) & 87.83  (267) & 85.48  (242) \\
&Adam                                                               & 85.86   (66) & 86.76   (52) & 86.55   (68) & 87.70  (108) & 86.29   (68) & 85.48   (73) \\
&RMSprop                                                            & 82.78   (38) & 87.40   (71) & 86.72   (48) & 83.98   (28) & 83.25   (41) & 86.08   (82) \\
\cmidrule{2-8}
%&\ourAcronym{} (10)                                                           & &  & &  & &  \\
%&\ourAcronym{} (30)                                                           & &  & &  & &  \\
%&\ourAcronym{} (50)                                                           & &  & &  & &  \\
&\ourAcronym{} (offline)                                                      & 85.94  (105) & 86.50   (69) & 85.52   (54) & 84.58   (50) & 84.15  (104) & 83.52  (89)  \\
\cmidrule{1-8}
\cmidrule{1-8}
\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{2-Layer MLP}}}
&SGD                                                                & 90.10 (3485) & 89.80 (1644) & 91.52 (3998) & 91.30 (3486) & 92.16 (4874) & 91.35 (3483) \\
&SGD +M09                                                           & 90.49  (565) & 91.39  (525) & 91.13  (400) & 90.36  (401) & 92.20  (833) & 91.39  (492) \\
&Adam                                                               & 88.00  (132) & 86.68   (64) & 88.39  (108) & 92.03  (173) & 90.49  (219) & 91.26  (138) \\
&RMSprop                                                            & 90.66  (160) & 90.40  (537) & 89.50  (392) & 84.79   (63) & 92.72  (348) & 90.10  (161) \\
\cmidrule{2-8}
%&\ourAcronym{} (10)                                                & &  & &  & &  \\
%&\ourAcronym{} (30)                                                & 92.46  (275) & 92.25  (252) & 92.54  (374) & 91.26  (206) & 91.90  (301) & 91.05  (304)  \\
%&\ourAcronym{} (50)                                                & &  & &  & &  \\
&\ourAcronym{} (offline)                                           & 90.57  (301) & 90.36  (181) & 91.22  (305) & 91.25  (256) & 90.70  (312) & 90.66  (226)  \\
\cmidrule{1-8}
\cmidrule{1-8}
\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{3-Layer MLP}}}
&SGD                                                                & 92.89 (5167) & 93.10 (6729) & 92.84 (5805) & 92.89 (5128) & 93.36 (4629) & 93.36 (6153) \\
&SGD +M09                                                           & 92.67  (576) & 93.06  (752) & 92.67  (902) & 92.07  (578) & 94.04  (934) & 92.29  (512) \\
&Adam                                                               & 88.09  (119) & 89.97  (155) & 91.30  (230) & 91.26  (513) & 91.39  (280) & 89.59  (273) \\
&RMSprop                                                            & 88.73  (180) & 91.00  (322) & 89.03  (250) & 88.90  (281) & 90.53  (514) & 92.33  (504) \\
\cmidrule{2-8}
%MMD  ()             &  &  &  &  & &  \\
%&\ourAcronym{} (10)                                                & &  & &  & &  \\
%&\ourAcronym{} (30)                                                & &  & &  & &  \\
%&\ourAcronym{} (50)                                                & 91.96  (632) & 93.40  (682) & 92.16  (738) & 92.03  (412) & 91.30  (602) & 92.97  (432)  \\
&\ourAcronym{} (offline)                                           & 92.29  (457) & 92.89  (827) & 93.36  (443) & 92.46  (403) & 93.14  (640) & 93.27  (696)  \\
\cmidrule{1-8}
\cmidrule{1-8}
\end{tabular}
}
\end{table*}

\cut{
\begin{table*}[t]
\centering
\caption{\textbf{Short Horizon Analysis}: RotatedMNIST with MLPs, test Accuracy/(training iteration) (\%) 3-Layer MLP } 
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{  l | c c c c c c}
\toprule
Method & 0 & 15 & 30 & 45 & 60 & 75 \\
\midrule
\ourAcronym{} (30)                                                & 91.13 (332)  & 91.22 (499)  & 89.80 (312)  & 91.39 (572)  & 90.70 (293)  & 91.39 (210)  \\
\ourAcronym{} (50)                                                & 91.96  (632) & 93.40  (682) & 92.16  (738) & 92.03  (412) & 91.30  (602) & 92.97  (432)  \\
\ourAcronym{} (70)                                                & 93.23 (500)  & 92.33 (427)  & 93.49 (480)  & 92.03  (361) & 92.46  (264) & 92.07  (331) \\
\ourAcronym{} (offline)                                           & 92.29  (457) & 92.89  (827) & 93.36  (443) & 92.46  (403) & 93.14  (640) & 93.27  (696)  \\
\midrule
\end{tabular}
}
\end{table*}
}

\cut{
\begin{table*}[t]
\centering    
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{ l | l | c c c c c c}
\toprule
&Method & 0 & 15 & 30 & 45 & 60 & 75 \\
\cmidrule{1-8}
\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{1-Layer MLP}}}
&SGD                                                                & 84.92 (1383) & 86.89 (1790) & 86.38 (1674) & 86.55 (1499) & 86.85 (1644) & 85.39 (1814) \\
&SGD +M09                                                           & 84.75  (192) & 86.50  (200) & 87.10  (223) & 87.10  (179) & 87.83  (267) & 85.48  (242) \\
&Adam                                                               & 85.86   (66) & 86.76   (52) & 86.55   (68) & 87.70  (108) & 86.29   (68) & 85.48   (73) \\
&RMSprop                                                            & 82.78   (38) & 87.40   (71) & 86.72   (48) & 83.98   (28) & 83.25   (41) & 86.08   (82) \\
\cmidrule{2-8}
%&\ourAcronym{} (50)                                                           & &  & &  & &  \\
&\ourAcronym{} (offline) k = 1                      & 85.94  (105) & 86.50  (69)  & 85.52   (54) &  84.58   (50) & 84.15  (104) & 83.52  (89)  \\
&\ourAcronym{} (offline) k = 5                      & 84.62  (543) & 85.05 (386)  & 85.35  (440) & 85.22   (418) & 84.02 (290) & 83.72 (504)  \\ 
&\ourAcronym{} (offline) k = 10                     & 84.58  (606) & 85.99 (491)  & 85.60  (605) &  85.73  (503) & 84.17  (235) & 83.98 (451) \\ 
&\ourAcronym{} (offline) k = 20                 & 85.86 (850) & 85.43 (637) & 86.38 (625) & 87.70 (733)  & 86.29 (494) & 85.22 (591) \\ 
\cmidrule{1-8}
\cmidrule{1-8}
\end{tabular}
}
\end{table*}
}
For clear illustration, we plot the performance trend change of learned optimisers according of the increase of the inner loop iteration. It can be noticed that for ...

\subsection{Optimiser learning for the Large scale problem}
\begin{itemize}
\item Need to plot the convergence rate graph here. 
\end{itemize}
We use LeNet and a group of dataset: MNIST, QMNIST, KMNIST, FashionMNIST, USPS, SVHN to conduct more challenging experiemtns to test the generalisation ability. \cut{Two meta-train and meta-test splitings are build from these datasets.} 
To adapt to the standard LeNet architeccture, all the images are resized to $28\time28$ with greyscale.
The gradient norm of the neural network increases alongside with the increase of the number of parameters. When the network come deeper and deeper, it is not appropriate to use gradient norm as the stopping criteria for the determination of convergence. In this section, we stop the training of the neural network, when the training loss is plateaued, which can be described as $||max(L_{t+\Delta}) - min(L_{t+\Delta})||_{1} \leqslant \beta, L_{t+\Delta} = \{l_t, l_{t+1}, ..., l_{t+\Delta}\}$

\begin{table*}[t]
\centering
\caption{\textbf{LeNet + MNIST family, test Accuracy(\%)}} 
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{ l | c c c c c c}
\toprule
Method & MNIST & QMNIST & KMNIST & FashionMNIST & USPS & SVHN \\
\midrule
SGD            & 96.44 $\pm$ 0.91 & 96.23 $\pm$ 0.73 & 87.61 $\pm$ 1.87 & 88.95 $\pm$ 1.43 & 92.73 $\pm$ 1.13 & 85.44 $\pm$ 1.22 \\
SGD+M          & 98.47 $\pm$ 0.16 & 97.21 $\pm$ 0.15 & 92.54 $\pm$ 0.62 & 86.44 $\pm$ 0.45 & 95.37 $\pm$ 0.24 & 86.26 $\pm$ 0.48  \\
Adam           & 98.49 $\pm$ 0.17 & 98.10 $\pm$ 0.33 & 93.20 $\pm$ 0.82 & 87.36 $\pm$ 0.55 & 93.68 $\pm$ 0.38 & 87.07 $\pm$ 0.61  \\
RMSprop        & 98.65 $\pm$ 0.21 & 98.30 $\pm$ 0.09 & 93.14 $\pm$ 0.87 & 87.45 $\pm$ 0.13 & 95.43 $\pm$ 1.06 & 87.01 $\pm$ 0.18  \\
\midrule
\ourAcronym{}  & 98.64 $\pm$ 0.12 & 98.41 $\pm$ 0.08 & 92.81 $\pm$ 0.33 & 87.72 $\pm$ 0.42  & 95.61 $\pm$ 0.70 & 87.59 $\pm$ 0.92   \\
\bottomrule
\end{tabular}
}
\end{table*}
\subsection{Cross Domain with Deep Model }
We have e
We studytwo sets of experiments to evaluate the performance of the proposed algorithm and the learned optimiser on a challenging meta train/test splittings. We deploy the base learning with the ResNet18 backbone. \textbf{Meta Train: QMNIST, FashionMNIST, SVHN, STL10}, \textbf{Homogeneous Meta-test, Cifar10} and \textbf{Heterogeneous Meta-test, Cifar100} 
\begin{table}[t]
\centering
\caption{Test performance on Cifar10 with ResNet18 with different optimisers} 
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{ l | c c c c}
\toprule
Method & SGD-M & Adam & AdamW  & \ourAcronym{}\\
\midrule
Accuracy & 95.01  & 94.07 & 94.49 & 93.70  \\
\bottomrule
\end{tabular}
}
\end{table}

\begin{figure*}[t]
\centering
\includegraphics[width=0.24\textwidth]{resnet18_cifar10_plot/res18_cifar10_training_acc.eps}
\includegraphics[width=0.24\textwidth]{resnet18_cifar10_plot/res18_cifar10_test_acc.eps}
\includegraphics[width=0.24\textwidth]{resnet18_cifar10_plot/res18_cifar10_training_loss.eps}
\includegraphics[width=0.24\textwidth]{resnet18_cifar10_plot/res18_cifar10_test_loss.eps}
\caption{Learning curve comparison of different optimiser on Cifar10 with ResNet18. From left to right: training accuracy, test accuracy, training loss, test loss}
\label{fig:resnet18_cifar10}
\end{figure*}

\cut{
\begin{figure}[t]
\centering
\includegraphics[width=0.49\columnwidth]{resnet18_cifar10_plot/res18_cifar10_training_acc.eps}
\includegraphics[width=0.49\columnwidth]{resnet18_cifar10_plot/res18_cifar10_test_acc.eps}
\includegraphics[width=0.49\columnwidth]{resnet18_cifar10_plot/res18_cifar10_training_loss.eps}
\includegraphics[width=0.49\columnwidth]{resnet18_cifar10_plot/res18_cifar10_test_loss.eps}
\caption{The optimisation trajecotries for solving the Rosenbrock function producded by different optimisers.}
\label{fig:resnet18_cifar10}
\end{figure}
}

\subsection{Ablation study}
To further understand the behaviour of the proposed algorithm, we study the effect of one component in the outer loop objective. 

\keypoint{Mahalanobis Matrix activation analysis}
\begin{figure}[t]
\centering
    \begin{minipage}[t]{.48\linewidth}
    \includegraphics[width=\linewidth]{mahalanobis_analysis/mahalanobis_activation_Frequence.eps}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.48\linewidth}
    \includegraphics[width=\linewidth]{mahalanobis_analysis/resnet18_cifar_idx_comparison__test.eps}
    \end{minipage} 
\end{figure}

\begin{table}[H]
\begin{tabular}{ l | c c c c}
\toprule
        Matrix & 0 & 1 & 2  & total\\
        \midrule
        Accuracy & 93.48  & 93.56 & 93.28 & 93.74  \\
        \bottomrule
        \end{tabular}
        \caption{Accuracy of the different Mahalanobis matrix} 
    \end{table}



























